Graph Pattern Matching for Dynamic Team Formation

Finding a list of k teams of experts, referred to as top-k team formation, with the required skills and high collaboration compatibility has been extensively studied. However, existing methods have not considered the specific collaboration relationships among different team members, i.e., structural constraints, which are typically needed in practice. In this study, we first propose a novel graph pattern matching approach for top-k team formation, which incorporates both structural constraints and capacity bounds. Second, we formulate and study the dynamic top-k team formation problem due to the growing need of a dynamic environment. Third, we develop an unified incremental approach, together with an optimization technique, to handle continuous pattern and data updates, separately and simultaneously, which has not been explored before. Finally, using real-life and synthetic data, we conduct an extensive experimental study to show the effectiveness and efficiency of our graph pattern matching approach for (dynamic) top-k team formation.

==> sec-opt.tex <==
\section{Optimization with Graph Filtering}
\label{sec-opt}

In this section, we propose graph filtering based optimization techniques to
enhance the algorithm proposed in Section~\ref{sec-topk}.

Our optimization techniques works for the following scenario.
We have a local data graph $G$ and a user specified positive integer $r$, and
we want to find top-$k$ group recommendations for each {\em online query}
$\langle Q, k\rangle$, where $Q$ is a pattern graph and $k$ is a positive
integer, \ie find the top-$k$ densest valid groups for $Q$ of $G$ \wrt $r$ for
each online query $\langle Q,k\rangle$.

The optimization is based on an idea of graph filtering: filter out the candidates that are not possible to contain results as early as possible. After executing top-$k$ offline process and before executing top-$k$ online process, we can employ a filtering process on $BL$ to remove the balls that are not possible to contain valid groups, which we refer to as false balls. And that will certainly reduce the execution time in finding out top-$k$ results. It contains a filtering offline preprocessing process over the set of balls in $BL$, and a filtering online process for each input query, in which we utilize an effective and efficient pruning strategy to remove false balls from $BL$ as many as possible. Finally, we can execute top-$k$ online process on the revised ball list $BL$.

In filtering offline process, we need to identify some pruning rules, which is usually executed based on features selected from candidates. In filtering online process, given a query graph, if there exists a feature that the query graph has while a data ball does not have, the data ball will be eliminated from the candidate set safely. \textcolor[rgb]{0.00,0.00,1.00}{TO be more CONCRETE!}


\subsection{Offline(\&online): Building Hybrid Star-feature Indices}

\stitle{Star-feature selection}

When deal with directed graphs, as we have seen in section~\ref{subsec-extsim}, graph simulation preserves the labels and the child relationship of a graph pattern in its match. When it comes to undirected graphs, graph simulation still preserves the label relationship, and preserves the neighbor relationship of a graph pattern in its match instead of child relationship in directed graphs. Therefore, we utilize the ``neighbor relationship" character as the pruning rule, and use the feature ``star" to represent the ``neighbor relationship" character. A star is a graph structure with a center node in the middle and a set of neighbor nodes adjacent with the center node. For each ball $\ball{v, r}$ in data graph $G$, and for each node $w$ in the ball, we construct one corresponding star-feature, eg..., so we get a set of star-features $F$ for each ball.

For all the balls $\ball{v, r}[1]$, $\ball{v, r}[2]$,...,$\ball{v, r}[n]$ in data graph $G$, we construct the corresponding feature sets $F[1]$,$F[2]$,...,$F[n]$. When a pattern graph comes, we construct the corresponding star-feature set $FP$ and compare it with $F[i]$ ($1\leq i\leq n$) of $\ball{v, r}[i]$. For each feature $fp$ in $FP$, if there exists a feature $f$ in $F[i]$ containing $fp$ as a substructure, then there may exist a matching result in $\ball{v, r}[i]$ and need further validation in the top-$k$ process. Otherwise, $\ball{v, r}[i]$ is pruned from candidate set safely.

In the above indices construction, for each ball $\ball{v, r}[i]$ ($1\leq i\leq n$) with $m_i$ nodes, we construct $m_i$ star-features. But it may be a waste of time and space to retrieve and store such lots of features, we can retrieve less features with stronger filtering power, making a balance between complexity and the pruning power. Therefore, We will improve this by adopting the next two star-feature selection strategies respectively.

Given a graph $H$, we want to select as few star-features as possible, which requires each star-feature to have strong pruning power and differ from other star-features obviously. This inspires us to think about the star minimization problem we will discuss in this section.

\etitle{Star minimization problem}. Given a graph $H(V_h, E_h)$, Star minimization problem is to select a set of star-features $F$ from $H$, with the union of edges of star-features in $F$ covering all the edges in $E_h$, while $|F|$ is minimized.

\begin{theorem}
\label{thm-star-mini-complexity}
Given a graph $H(V_h, E_h)$, and a positive integer $\xi$, it is \NP-complete to determine whether there exists a star-feature set $F$ with the union of edges of star-features in it covering all the edges in $E_h$, and the number of items in $F$ is no larger than $\xi$.
\end{theorem}

\textbf{Approximation hardness:}

\begin{theorem}
\label{thm-star-mini-complexity}
There exists a factor 2 approximation algorithm for the Star minimization problem.
\end{theorem}

We present the 2-approximation algorithm in Fig.~\ref{star-min-alg}.

\begin{figure}[tb!]
\vspace{2ex}
\begin{center}
{\small

\myhrule \vspace{-2ex}
\mat{0ex}{
\sstab {\sl Input:\/} Graph $H(V_h$, $E_h)$.\\
{\sl Output:\/} The set of star-feature $F$ of $H$.\\
\bcc \quad $C:=\emptyset$; $F:=\emptyset$;\\
\icc \quad $H'(V_h', E_h'):=H(V_h, E_h)$;\\
\icc \quad while $E_h'$ is not empty do\\
\icc \quad\quad pick any $(u, v) \in E_h'$;\\
\icc \quad\quad $C:=C \cup \{(u, v)\}$;\\
\icc \quad\quad remove all edges incident to either $u$ or $v$ in $H'$.\\
\icc \quad for each node $w$ in $C$ do\\
\icc \quad\quad construct star feature $f$ takes $w$ as the center node in $H$;\\
\icc \quad\quad $F:=F \cup f$;\\
\icc return $F$;\\

}
\vspace{-2.5ex} \myhrule
}
\end{center}
\vspace{-4ex}
\caption{Algorithm StarMin} \label{star-min-alg}
\vspace{-3ex}
\end{figure}

There is another scene that users have the chance to specify a number, indicating how many star-features necessarily to be selected from the given graph. It requires the fixed number of star-features we select should have strong pruning power, representing as much structural information as possible. This is another feature selection strategy we will consider next.

\etitle{$K$-star coverage maximization problem}. Given a graph $H(V_h, E_h)$ and a user specified integer $K$, $K$-star coverage maximization problem is to select a set of star-features $F$ from $H$, with the union of edges of star-features in $F$ covering as many edges as possible in $E_h$.

\begin{theorem}
\label{thm-k-star-max-complexity}
Given a graph $H(V_h, E_h)$, two positive integers $K$ and $\xi$, it is \NP-complete to determine whether there exists a $K$ item star-feature set $F$, in which the number of the union of edges of the star-features is no smaller than $\xi$.
\end{theorem}

\textbf{Approximation hardness:}

\begin{theorem}
\label{thm-star-mini-complexity}
There exists a 3/4-approximation algorithm for the $K$-star coverage maximization problem.
\end{theorem}

We present the 3/4-approximation algorithm in Fig.~\ref{k-star-max-alg}.

\begin{figure}[tb!]
\vspace{2ex}
\begin{center}
{\small

\myhrule \vspace{-2ex}
\mat{0ex}{
\sstab {\sl Input:\/} Graph $H(V_h$, $E_h)$, a positive integer $K$.\\
{\sl Output:\/} The set of star-feature $F$ of $H$.\\
\bcc \quad $C:=\emptyset$; $F:=\emptyset$;\\
\icc \quad for $i=1$ to $K$ do\\
\icc \quad\quad select node $v$ from $H$ while the number of edges $C \cup \{v\}$ \\covers is maximized ;\\
\icc \quad for each node $w$ in $C$ do\\
\icc \quad\quad construct star feature $f$ takes $w$ as the center node in $H$;\\
\icc \quad\quad $F:=F \cup f$;\\
\icc return $F$;\\

}
\vspace{-2.5ex} \myhrule
}
\end{center}
\vspace{-4ex}
\caption{Algorithm K-StarMax} \label{k-star-max-alg}
\vspace{-3ex}
\end{figure}

\textcolor[rgb]{1.00,0.00,0.00}{\textbf{Remark.}
Establish the filtering power standards of star features.
1. Covering more edges
2. Covering more nodes}

\stitle{Hybrid Star Index Structure}.

In last section, for each ball $\ball{v, r}$ in data graph $G$, we construct a star-feature set $F$. When a pattern graph $P$ comes, we construct the corresponding star-feature set $FP$ and compare it with $F$. If $P$ and $\ball{v, r}$ are matched via extended graph simulation, for each star-feature $fp$ in $FP$, there must exist a corresponding $f$ in $F$ such that $fp$ is a substructure of $f$. That is, the local structure represented by $fp$ in $P$ must be preserved by $f$ in $\ball{v, r}$. Therefore, we need to check all the star-features in $FP$ to see whether there exist the corresponding structures in $\ball{v, r}$ preserving the local structure, such that we can remove the false positives in the filtering process. However, a question arises, as the structure comparison operation is expensive, how can we implement the checking process efficiently? In this section, we propose Hybrid-Star-Index-Structure to encode the local information of star-features selected in last step, improving the speed of comparison operation in filtering process to a large extent.

\etitle{Index structure for small label data graph}

We will present a encoding method, for the case when the number of labels appearing in data graph is small, which encodes the local information taken by the star to numerical space. For each star-feature, it generates a bit string with fixed-length, called \textbf{Star-fingerprint}, providing a convenient way to execute filtering process just on those star fingerprints, with no need referring to the originally star-feature structures.

\begin{definition} {\textbf{Star-fingerprint.}}
\label{def-ind-str-small-label}
Given a data ball $\ball{v, r}$ in $G$ and the corresponding star-feature set $F=\{s_1, s_2,..., s_m\}$ of the ball, for any star-feature $s_i$ $(1 \leq i \leq m)$ in $F$, the star-fingerprint $starfig(s_i)$ of $s_i$ is a two-tuples $<C,N>$, where $C$ denotes the center node with id and label of star $s_i$, and $N$ is a length-$L$ bit string, denoting the neighbor labels, where $L$ is the total number of labels appearing in $G$, and each bit indicates the appearance of the corresponding label in neighbors.
\end{definition}

By Definition~\ref{def-ind-str-small-label}, in the two-tuples $<C,N>$, $C$ is to denote the center node and $N$ is to denote the neighbor labels of center node. For each distinct neighbor label, it sets the corresponding position element in the bit string to 1, indicating there exists at least one neighbor node carrying the label. For example, Fig~\ref{fig-starfingerprint-example} shows an example on how to generate the star-fingerprint.

\begin{figure}[tb!]
\begin{center}
\includegraphics[scale=0.4]{./fig/star-fingerprint.eps}
\caption{Star Fingerprint}
\label{fig-starfingerprint-example}
\end{center}
\end{figure}


\begin{prop}
\label{prop-star-fingerprint-condition}
Given a data graph $G$, a pattern graph $P$, and a positive integer $r$, if subgraph $G_{s}$ of $G$ is a {\em valid group} for $P$ \wrt $r$, then for each vertex $v$ in $P$, whose star-feature is $s_v$, and star-fingerprint $starfig(s_v)$ is $<C_p,N_p>$, there must exist a matched vertex $u$ in $G_{s}$, whose star-feature is $s_u$, and star-fingerprint $starfig(s_u)$ is $<C_g,N_g>$. The two star fingerprints must satisfy the following two conditions: 1)$l(C_p)=l(C_g)$; 2)$N_p \wedge N_g = N_p$.
\end{prop}

By proposition~\ref{prop-star-fingerprint-condition}, assume $G_{s}$ of $G$ is a {\em valid group} of $G$ for $P$. A vertex $v$ in $P$ is matched with a vertex $u$ in $G_{s}$. The vertices $v$ and $u$ are matched via extended graph simulation requires the two conditions hold, because according to extended graph simulation, the labels of $v$ and $u$ must be same (condition 1); and the labels of neighbors of $v$ must be a subset of the labels of neighbors of $u$ (condition 2).

\begin{theorem} {\textbf{Star-fingerprint Pruning 1.}}
\label{thm-star-fingerprint-pruning}
Given a data ball $\ball{v, r}$ of $G$ and a pattern graph $P$, for each vertex $v$ in $P$ with star-feature $s_v$, if there exists no vertex $u$ in $\ball{v, r}$ with star-feature $s_u$, where fingerprints $starfig(s_v)$ and $starfig(s_u)$ satisfy the two conditions in proposition~\ref{prop-star-fingerprint-condition}, there must exist no {\em valid group} in $\ball{v, r}$ of $G$ for $P$.
\end{theorem}

Apparently, this is a feature to feature comparison, and we can prune the set of balls cannot have a valid group inside quickly according to the pruning rule proposed in  theorem~\ref{thm-star-fingerprint-pruning}. It has a good performance when the length-$L$ bit string is short, as the comparison between two fingerprints can be executed by a bitwise AND operation in $O(L)$ time.

\etitle{Index structure for large label data graph}

When the number of labels appearing in data graph is really large, it is inconvenient to adopt the star-fingerprint method to represent the star feature. That is, when $L$ is large, adopting the $L$-length bit string is not efficient for the star feature expression and feature to feature comparison. Therefore, we will present another encoding method for representing star-features extracted from the data graph with large number of labels. For each star-feature, it generates a bit string with specified length, called \textbf{Star-bloomfilter}. This is a method based on the space-efficient data structure \textbf{bloom filter}, both reducing the storage space requirement and improving filtering speed.

A Bloom filter is a length-$X$ bit string. Given a set of elements and a query item, the bloom filter is used to check whether the query element is contained in the set. There are also $k$ predefined hash functions, each of which hashes an item to one of the $X$ positions with a uniform random distribution. For each element, feed it to each of the $k$ hash functions to get $k$ bit positions, and set the bits at all these positions to 1. To query whether there exists an element in the set, just feed it to each of the $k$ hash functions to get $k$ bit positions, check whether all these bits are set to 1. If there exists any position the bit is 0, then the element is not in the set. If it were, then the element has a high probability in the set, but there may exist ``false positives" due to collisions in hash functions. By this observation, given a query graph and a data ball, when executing the feature to feature comparison, say $f$ in data ball and $fp$ in query graph, we can use a bloom filter to encode the neighbor label set of $s$, and check for each neighbor label in $fp$, whether it is contained in $s$ by checking the bloom filter. Finally, we can filter out a set of unmatched data balls in advance.

\begin{definition} {\textbf{Star-bloomfilter.}}
\label{def-ind-str-large-label}
Given a data ball $\ball{v, r}$ in $G$ and the corresponding star-feature set $F=\{s_1, s_1,..., s_m\}$  of the ball, for each star-feature $s_i$ $(1 \leq i \leq m)$ in $F$, the star-bloomfilter $starblm(s_i)$ of $s_i$ is a two-tuples $<C,N>$, where $C$ denotes the center node with id and label of star $s_i$, and $N$ is a length-$X$ bit string bloom filter, denoting the neighbor labels, where $X$ is a user specified number.
\end{definition}

By Definition~\ref{def-ind-str-large-label}, in the two-tuples $<C,N>$, $C$ is to denote the center node and $N$ is to denote the neighbor labels of center node. For each distinct neighbor label, by the set of $k$ hash functions, it sets the corresponding $k$ position element in the bit string to 1, indicating there exists at least one neighbor node carrying the label. For example, Fig~\ref{fig-bloomfilter-example} shows an example on how to generate the star-bloomfilter.

\begin{figure}[tb!]
\begin{center}
\includegraphics[scale=0.4]{./fig/star-bloomfilter.eps}
\caption{Star Bloomfilter}
\label{fig-bloomfilter-example}
\end{center}
\end{figure}


\begin{prop}
\label{prop-star-bloomfilter-condition}
Given a databall graph $G$, a pattern graph $P$, and a positive integer $r$, if subgraph $G_{s}$ of $G$ is a {\em valid group} for $P$ \wrt $r$. Then for each vertex $v$ in $P$, whose neighbor label set is $lset$, there must exists a matched vertex $u$ in $G_{s}$, whose star-feature is $s_u$, and star-bloomfilter $starblm(s_u)$ is $<C_g,N_g>$. They must satisfy the following two conditions: 1)$l(v)=l(C_g)$; 2)for each item in $lset$, feed it to each of the $k$ hash functions to get $k$ bit positions in $N_g$, all the $k$ bits are set to 1.
\end{prop}

By proposition~\ref{prop-star-bloomfilter-condition}, assume $G_{s}$ of $G$ is a {\em valid group} of $G$ for $P$. A vertex $v$ in $P$ is matched with a vertex $u$ in $G_{s}$. The vertices $v$ and $u$ are matched via extended graph simulation requires the two conditions hold, because according to extended graph simulation, the labels of $v$ and $u$ must be same (condition 1); and the labels of neighbors of $v$ must be a subset of the labels of neighbors of $u$ (condition 2).

\begin{theorem} {\textbf{Star-bloomfilter Pruning 2.}}
\label{thm-star-bloomfilter-pruning}
Given a data ball $\ball{v, r}$ of $G$ and a pattern graph $P$, for a vertex $v$ in $P$, if there exists no vertex $u$ in $\ball{v, r}$ with star-feature $s_u$, where $v$ and bloomfilter $starblm(s_u)$ of $u$ satisfy the two conditions in proposition~\ref{prop-star-bloomfilter-condition}, there must exist no {\em valid group} in $\ball{v, r}$ of $G$ for $P$.
\end{theorem}

Obviously, when the label number $L$ is small, we can use the length-$L$ star-fingerprint bit string, in which each bit represents a label directly; when the label number $L$ is large, we can reduce the storage space of a star feature encoding string significantly by utilizing bloomfilter data structure, from length-$L$ star-fingerprint bit string to length-$X$ star-bloomfilter bit string by using hash functions.

\textcolor[rgb]{1.00,0.00,0.00}{\textbf{Remark.}
Probability analyze for bloomfilter}

\stitle{Index structure for the whole data ball(Graph Code)}.

The above ``star to star" pruning process is time-consuming. We will next provide some quick pruning rules based on graph code. Such that when a query graph comes, we could execute ``graph to graph" filtering first, quickly pruning out the set of candidates obviously cannot match with query graph in the first filtering phase, and then employ the ``star to star" filtering with stronger pruning capability. We know that extended graph simulation preserves label and number relationship between data graph and pattern graph, so we can take those two characters as a pruning rule. In the first filtering phase, we could efficiently eliminate the set of candidates which violate the label and number constraints taken by pattern graph. Then in the second phase, we further check whether the candidates preserve the structural constraints taken by pattern graph by making the ``star to star" validation.

In this section we will present a encoding method for data balls, which encodes the label and node number information taken by the ball to numerical space. For each data ball, it generates a list , called \textbf{Graph-code}.

\begin{definition} {\textbf{Graph-code.}}
\label{def-ind-graph-code-arr}
Given a data ball $\ball{v, r}$ of $G$, the graph-code $B$ of $\hat{G}$ is a list. Each item in the list is a two-tuple $<Lab, Num>$, where $Lab$ indicates there exists at least one node in $\hat{G}$ labeled with $Lab$, and $Num$ denotes there are $Num$ nodes carrying the label $Lab$.
\end{definition}

Fig.~\ref{fig-graphcode-example} shows an example on how to generate the Graph code. \textcolor[rgb]{0.00,0.00,1.00}{MORE examples, combine with star-feature.}

\begin{figure}[tb!]
\begin{center}
\includegraphics[scale=0.5]{./fig/graph-code.eps}
\caption{Graph Code}
\label{fig-graphcode-example}
\end{center}
\end{figure}

\begin{prop}
\label{prop-graph-code-condition}
Given a data graph $G$, a pattern graph $P$, and a positive integer $r$, if subgraph $G_{s}$ of $G$ is a {\em valid group} for $P$ \wrt $r$, and is contained in $\ball{v, r}$. The graph code $B_p$ of $P$ and the graph code $B_g$ of $\ball{v, r}$ must satisfy the following conditions:  for each item $<Lab_p,Num_p>$ in $B_p$, there must exist the corresponding item $<Lab_g,Num_g>$ in $B_g$ with 1) $Lab_p=Lab_g$, and 2) $Num_p \leq Num_g$.
\end{prop}

By proposition~\ref{prop-graph-code-condition}, assume $G_{s}$ of $G$ is a {\em valid group} of $G$ for $P$, and is contained in $\ball{v, r}$. $P$ and $G_{s}$ in $\ball{v, r}$ match via extended graph simulation requires the above conditions hold. Because according to extended graph simulation, each label $l$ contained in $P$ must be contained in $\ball{v, r}$, and the number of nodes labeled with $l$ must satisfy the lower bound requirement in $P$.

\begin{theorem} {\textbf{Graph-code Pruning 3.}}
\label{thm-graph-code-pruning}
Given a data ball $\ball{v, r}$ of $G$ and a pattern graph $P$, if there exists no subgraph $G_s$ in $\ball{v, r}$, where graph-code $B_p$ of $P$ and $B_g$ of $\ball{v, r}$ satisfy the conditions in proposition~\ref{prop-graph-code-condition}, there must exist no {\em valid group} in $\ball{v, r}$ for $P$.
\end{theorem}

Apparently, this is a graph to graph comparison, and we can efficiently prune out the set of candidates which violate the label and number constraints taken by pattern graph. It has a good performance as the comparison between two lists can be executed by linear scanning operation in $O(l_p+l_g)$ time ($l_p$ is the number of labels in $P$, and $l_g$ is the average number of labels among all the balls? Does average work?).

\subsection{(Online:) Improving Early Termination}

In order to accelerate the speed of finding match results, we combine the top-k early termination process with filtering method. Given a data graph $G$, we first generate the set of balls $ball_1$, $ball_2$,..., $ball_n$, with upper bounds $U_1$, $U_2$,..., $U_n$ ($U_1 \leq U_2,..., \leq U_n$ ), and then extract features from each ball and construct the indices. When given a pattern graph $P$, we first extract the set of features and establish the indices for $P$, and then perform the filtering process with the indices, eliminating the set of balls that cannot have matched subgraphs inside \wrt $P$. Then we execute the top-$k$ procedure, finding out the set of matches. The main steps are as below.

\stitle{Step1: Data graph Preprocess}. Generate the set of balls with upper bounds and feature indices.

\stitle{Step2: Pattern graph preprocess}. Extract features and establish index.

\stitle{Step3: Graph Code (node label and node number) filtering}. First filtering phase according to graph code pruning rule.

\stitle{Step4: Star-feature filtering}. Second filtering phase according to star-feature pruning rule.

\stitle{Step5: Top-k process}. Find out top-k match results of $G$.

\subsection{Putting Things Together}

title for last section 

==> sec-related.tex <==
\section{Related Work}
\label{sec-related}

%We categorize the related work as follows.


\stitle{Team formation}. There has been a host of work on team formation by minimizing the communication cost of team members, defined with the diameter, density, minimum spanning tree, Steiner tree, and sum of pairwise member distances among others~\cite{Lappas09,Kargar11,ArisLuca12,GajewarS12,realTeamForm13,SamikKVM12,LiTongCao15}.
Similar to~\cite{Kargar11}, we are to find the top-$k$ teams. However,
\cite{Kargar11} adopted Lawler's procedure \cite{Lawler1972}, which makes it hard to work on large data graphs. We also adopted {\em density}  as the communication cost, which shows a better performance~\cite{GajewarS12}. However, we further require that all team members are {\em close to each other} (located in the same balls), along the same lines as~\cite{Lappas09,Kargar11}.  Moreover, graph pattern matching has been used to search single experts, instead of a team of experts~\cite{FanWWXin13}. Different from these work, we introduce {\em structural constraints}, in terms of graph pattern matching~\cite{FanLMTWW10,MaCFHW14}, into team formation.

\eat{Team formulation with minimum communication cost in  terms of the diameter and minimum spanning tree was firstly studied in~\cite{Lappas09},
followed by

Afterwards, authors of~\cite{Kargar11,Kargar11,GajewarS12,SamikKVM12} extended and proposed new communication cost metrics or incorporated more constraints. \cite{GajewarS12,realTeamForm13} incorporated the number requirements for each required skill considering real-life factors, \cite{SamikKVM12} incorporated constraints ensures that no user is overloaded by the task assignment, and \cite{LiTongCao15} proposed the team member replacement problem to efficiently find a good candidate to replace a unavailable team member.




 simply maximizing density may return a quite large team and not practical in real life. We not only require the density to be large, but also require the distance between team members to be closed, as ~\cite{Lappas09,Kargar11} do.


  and~\cite{realTeamForm13},
 we incorporate the density metric as the communication cost, and the capacity constraint into


 while the others are devoted to find only one best team. However, the adaption of Lawler's


Our work differs from the prior work in the following. By adopting graph pattern matching semantic for team formation, (1) we can assign structural constraints between different skills, while ~\cite{Lappas09,Kargar11,realTeamForm13} only require the diameter or MST or the sum of distance between members of the team to be small, which can all be ensured by our model(the diameter bound in $r$-simulation semantic).

(2) We find top-$k$ best teams which is same with ~\cite{Kargar11}, while the others are devoted to find only one best team. However, the adaption of Lawler's procedure to find top-$k$ answers ~\cite{Kargar11} adopted prohibited it to execute on large data graphs. Because it execute $k$ rounds algorithms to find $k$ answers.

(3) We adopted density as proposed in ~\cite{GajewarS12} as our communication cost metric to rank for top-$k$ results. As illustrate by them, the density based communication cost is thus performing better than the previous. However, simply maximizing density may return a quite large team and not practical in real life. We not only require the density to be large, but also require the distance between team members to be closed, as ~\cite{Lappas09,Kargar11} do.

(4) We can assign upper and lower bound for each required skill, at this point, closer to our work is ~\cite{realTeamForm13}, however, it cannot satisfy other requirements.....

(5) A common shortcoming is that previous algorithms cannot execute on large data graphs which is essential in the big data era.

Closer to this work is ~\cite{FanWWXin13}, they have adopted graph pattern matching semantic to search for experts satisfying topology constraints. However, they could not find a team of experts for a given task.


}



\stitle{Graph pattern matching}. Recently, {\em graph simulation} \cite{infsimu95} and its extensions have been introduced for graph pattern matching~\cite{FanLMTWW10,FanLMTW11,MaCFHW14,Guanfeng15}, in which {\em strong simulation} introduces duality and locality into simulation~\cite{MaCFHW14}, and shows a good balance between its computational complexity and its ability to preserve graph topology.
$R$-simulation proposed in this work is an extension of strong simulation on undirected graphs with capacity constraints on pattern graphs.


\eat{
Closer to our work is ~\cite{MaCFHW14}. It proposed strong simulation, imposing two additional constraints on graph simulation: duality and locality. It is capable of capturing the topology in graph pattern matching and can be determined in cubic time.

, via subgraph isomorphism~\cite{Ullmann76}, an \NP-complete problem. To lower its complexity, various extensions of graph simulation have been considered instead~\cite{FanLMTWW10,FanLMTW11,MaCFHW14,Guanfeng15}. Graph simulation can be determined in quadratic time. However, the low complexity may cause the extended notions fail to capture the topology of graphs, and yield false matches or too large a match relation. Closer to our work is ~\cite{MaCFHW14}. It proposed strong simulation, imposing two additional constraints on graph simulation: duality and locality. It is capable of capturing the topology in graph pattern matching and can be determined in cubic time. This work differs from strong simulation in that we combine capacity bounds on pattern nodes to find matches satisfying the capacity requirements.
}



\stitle{Incremental computations}. Incremental algorithms (see \cite{inc-survey} for a survey) have proven usefulness in a variety of areas,
and have been studied for both graph pattern matching~\cite{FanLMTWW10,FanWW13-tods} and team formation \cite{ArisLuca12}.
However, \cite{FanLMTWW10,FanWW13-tods} only consider data changes,
and \cite{ArisLuca12} only consider continuous coming new tasks. In this work, we both deal with pattern and data updates for $r$-simulation, and allow both node/edge insertions and deletions, which is a much more general setting that has not been studied in \cite{ArisLuca12,FanLMTWW10,FanWW13-tods}.



\eat{
, and
For graph pattern matching problem, ~\cite{FanLMTWW10,FanWW13-tods} have proposed incremental algorithms dealing with data changes defined in terms of graph simulation, bounded simulation and subgraph isomorphism.


%\cite{FanWW2014} investigated the issue to answer graph pattern queries using graph pattern views.
%For team formation problem, \cite{GastonMarie05} studied the team formation problem on multi-agent networks in a setting where agents could adapt their network connectivity.
\cite{ArisLuca12} proposed the online algorithms that assemble teams to deal with continuous coming tasks. team data inc.


Our work differs from the prior work in the following.
(1) \cite{FanLMTWW10,FanWW13-tods} focused on dynamic computing strategies only concerning with data changes, while we provided a unified framework to deal with both data and pattern changes.
(2) For pattern change issue, \cite{FanWW2014} focused on accelerating the process to answer new queries with stored graph views, which are not capable to handle pattern changes.
%\cite{ArisLuca12} focussed more on the load balancing aspect when dealing with a series of tasks. While we focus on immediately answering queries of users with given pattern changes to the original patterns.
(3) \cite{FanLMTWW10,FanWW13-tods} have proved there exist bounded algorithms for single-data-edge deletion updates based on conventional incremental algorithms. However, existing approaches based on conventional incremental algorithms are proved unbounded when pattern incremental is concerned for any pattern update. Thus, we proposed a partition based framework comes with theoretical bounds in terms of \affballsx and \affballaccs that are essential for any incremental algorithms.
}


\stitle{Top-k queries}. Although top-$k$ queries (see~\cite{IlyasBS08} for a survey) have been investigated for both graph pattern matching and team formation~\cite{FanWW2013,Kargar11}.
However, to our knowledge, neither team formation nor graph pattern matching  has been studied in a dynamic setting for top-$k$ queries.


\eat{
There has been works exploring top-$k$ query answering in both graph pattern matching and team formation~\cite{FanWW2013,Kargar11}.
\cite{FanWW2013} studied the diversified top-$k$ graph pattern matching problem defined in terms of simulation.
\cite{Kargar11} designed a procedure to find top-$k$ teams, which is an adaption of Lawler's procedure~\cite{Lawler1972} for calculating the top-$k$ answers to discrete optimization problems.
This work differs from them in that besides finding top-$k$ teams in a static case, we consider finding top-$k$ teams in a pattern and data incremental manner.
Closer to this work is \cite{EVMK12}, which devoted to discover top-$k$ dense subgraphs in a stream of graphs.
It proposed a procedure with early termination property, a superior property which can accelerate the top-$k$ computing process.
However, they utilize a sliding window to find top-$k$ dense subgraphs only contained in the window, such that their top-$k$ procedure is similar with the static case.
It is difficult to use early termination for incremental algorithms. We define the {\em early return property}, an analogy to the early termination property for traditional top-$k$ algorithms and prove that our dynamic framework pertains this property.
}



\eat{

\stitle{Team formulation}. finding a team of exports
group recommendations
\stitle{Keywords on Graphs}.
\stitle{Graph pattern matching}.
Subgraph Isomorphism; Graph Simulation; Dual Simulation; strong simulation.
\stitle{Graphs density}.
\stitle{Diversity}.

\stitle{Graph pattern matching}.
Graph pattern matching is often defined according to subgraph isomorphism~\cite{Aggarwal10,Galla06}, an \NP-complete problem. However, it is too restrictive to catch sensible matches in most cases, as it requires match subgraphs to have exactly the same topology as the pattern graph. Subsequently, to reduce the time complexity, graph simulation~\cite{ccs} has been adopted for pattern graph matching which can be determined in quadratic time. It devotes to preserve the child relationship of pattern graph, but it may fail to capture the topology of graphs and yield false matches or too large a match relation. To rectify these problems, strong simulation~\cite{MaCFHW11} imposes two additional constraints on graph simulation: the duality to preserve both parent and child relationships, also referred to as dual simulation~\cite{MaCFHW11}, and the locality to eliminate excessive matches. It is capable of capturing the topology in graph pattern matching and can be determined in cubic time.

\stitle{Team formulation}.
Lappas et al.~\cite{Lappas09} is the first to consider team formulation problem while minimizing the communication cost. By formalizing communication cost as diameter and the total weights of minimum spanning tree(MST) induced by the team, Lapps et al have proved the problem is \NP-hard, and they have proposed an approximation algorithms for minimizing the diameter with a guarantee 2 and a greedy algorithm with no approximation ratio for MST. Authors of~\cite{Kargar11} proposed a new communication cost function of minimizing the sum of distances between each pair of skill holders and provided a 2-approximation algorithm. They also introduced the problem of finding a team of experts with a leader while considering another new communication cost function of minimizing the the sum of distance between the leader and each of the skill holders in the team. Authors of~\cite{GajewarS12} generalized this problem to the case where for each required skill, multiple  experts possessing the skill are desired.
%\cite{Chengte10} utilized MST as the metric of communication cost, but they have proposed algorithms with no approximation ratio.
In \cite{GajewarS12}, density based measures are used as objectives, they have proposed a 3-approximation algorithm for single skill team formation problem(sTF), and  greedy algorithm with no approximation ratio for multiple skill team formation problem(mTF).

\stitle{Graphs density}.
As mentioned above, \cite{GajewarS12} has utilized density as a measure of collaborative compatibility, and the problem of finding densest subgraphs has been well-studied these years. Given a undirected data graph, finding a subgraph with maximum density~\cite{Goldberg84} can be solved optimally in polynomial time. However when there is a size constraint specified, the densest-k-subgraph problem, namely, finding a densest subgraph with exactly $k$ vertices becomes \NP-hard~\cite{FeigeML01,FeigePK01}. The algorithm developed by Feige et al. achieves the best approximation ratio for now~\cite{FeigePK01}. Andersen et al~\cite{Andersen09} considered the problem of finding dense subgraphs with specified upper and lower bounds on the number of vertices, the densest-at-least-k-subgraph (Dalks) problem and the densest-at-most-k-subgraph (Damks) problem. Khuller et al~\cite{Khuller09} have shown that Dalks is \NP-complete. Andersen et al have shown that Damks is nearly as hard to approximate as Dks and gave constant factor approximation algorithms for Dalks.

}

